Interpretable Anomaly Detection with Mondrian P{\'o}lya Forests on Data Streams

Anomaly detection at scale is an extremely challenging problem of great practicality. When data is large and high-dimensional, it can be difficult to detect which observations do not fit the expected behaviour. Recent work has coalesced on variations of (random) $k$\emph{d-trees} to summarise data for anomaly detection. However, these methods rely on ad-hoc score functions that are not easy to interpret, making it difficult to asses the severity of the detected anomalies or select a reasonable threshold in the absence of labelled anomalies. To solve these issues, we contextualise these methods in a probabilistic framework which we call the Mondrian \Polya{} Forest for estimating the underlying probability density function generating the data and enabling greater interpretability than prior work. In addition, we develop a memory efficient variant able to operate in the modern streaming environments. Our experiments show that these methods achieves state-of-the-art performance while providing statistically interpretable anomaly scores.

==> mondrian-polya-tree.tex <==
% We introduce the \MPT: a combination of both the Mondrian Tree constructions
% introduced by \cite{lakshminarayanan2014mondrian} and the \PTree{} models
% given in [citation].
% The generative process for constructing such a tree is given in Algorithm
% (INSERT ALGORITHM).
% The classical Mondrian Forest easily admits online updates which enables its
% use in an online fashion.
% We complement this by showing that deletions for the the Mondrian Forest are
% also permissible, and consequently the Mondrian Forest can be used either on a
% stream of data or with a windowed approach.
% A crucial observation is that we can pair the Mondrian Forest with \PTree in a
% non-trivial fashion.
% To do so, we introduce \emph{pseudolevels} in the tree corresponding to two
% operations: \texttt{split} and \texttt{restrict}.
% The \texttt{split} operation is ...
% The \texttt{restrictin} operation is...
% Another strength of the \MPT{} is that the posterior parameters can be built in
% a single pass over the input as the data is observed.

% We need to distinguish between two types of leaves:
% \begin{itemize}
%   \item{\emph{Observation leaves:} Any leaf formed from cuts performed on the
%   observed data which contain two or more datapoints}

%   \item{\emph{Restriction leaves:} Leaves formed either when a cut on the
%   observations would isolate a point, or in a region where no observations are
%   made {\emph in the building stage}.
%   As such these leaves contain 0 or 1 datapoints during the building of the
%   tree.}
% \end{itemize}

% A crucial difference between our work and prior work on random forests for
% anomaly detection is the introduction of a probabilistic model.
% This allows flexibility in the tree generation process as the underlying
% dynamics of the \PTree{} enable us to learn properties of the distribution even
% when the data does not suit `natural' interpretations of how anomalies should
% be found in a tree.
% Specifically, consider the following example: there are two clusters of points
% $U,V$ with $|U| \gg |V| = 2$ which are separated sufficiently far apart so that
% the two points in $V$ are clearly anomalies given the dataset
% $\mathcal{D} = \{ U,V \}$.
% Further suppose that the the two points $v_1,v_2 \in V$ are located
% infinitesimally close to each other and that a tree sampled over $\mathcal{D}$
% separates $U$ from $V$; that is, $V$ is entirely stored in say the left child of
% the root node and $U$ entirely in the right child.
% This example motivates the scoring function used in \rrcf{} but it also
% demonstrates that a na\"ive combination of \rrcf{} and Mondrian Trees would not
% work.
% Since $v_1$ and $v_2$ are so close together, the linear dimension for their
% bounding box is exceptionally small.
% Consequently, we face the paradox of having two points which are clearly
% anomalous so are easily separated in the first cut, but the would take an
% unbounded amount of time to separate in the Mondrian Forest setting.
% As a result, either the two points are not separated and they occur very high
% in the tree as the exponential clock runs out of time, or they are separated
% and their weighted depth is very large, so they appear very low in the tree.
% This suggests that using depth as a proxy for being an anomaly could be flawed.



% \paragraph{High Level Interpretation}
% The setting is as for the \PTree{}, however we note that there are now two
% distinct splits.
% We distinguish between these parameters by $\chi_0, \chi_1$ for the Beta
% parameters determined by the cuts to generate the random tree, and the
% parameters used for `restricting' to the areas in which data is observed:
% $\rho_0, \rho_1$.

